Data-Driven Solvers for Strongly Nonlinear Material Response

This work presents a data-driven magnetostatic finite-element solver that is specifically well-suited to cope with strongly nonlinear material responses. The data-driven computing framework is essentially a multiobjective optimization procedure matching the material operation points as closely as possible to given material data while obeying Maxwell's equations. Here, the framework is extended with heterogeneous (local) weighting factors - one per finite element - equilibrating the goal function locally according to the material behavior. This modification allows the data-driven solver to cope with unbalanced measurement data sets, i.e. data sets suffering from unbalanced space filling. This occurs particularly in the case of strongly nonlinear materials, which constitute problematic cases that hinder the efficiency and accuracy of standard data-driven solvers with a homogeneous (global) weighting factor. The local weighting factors are embedded in the distance-minimizing data-driven algorithm used for noiseless data, likewise for the maximum entropy data-driven algorithm used for noisy data. Numerical experiments based on a quadrupole magnet model with a soft magnetic material show that the proposed modification results in major improvements in terms of solution accuracy and solver efficiency. For the case of noiseless data, local weighting factors improve the convergence of the data-driven solver by orders of magnitude. When noisy data are considered, the convergence rate of the data-driven solver is doubled.

==> coax_cable.tex <==
\begin{figure}[htb]
	\centering
	{\includegraphics[width=0.3\textwidth]{figures/coax_cable/standalone_fig_tube.pdf}} 
	\caption{Coaxial cable}
	\label{fig:coax_cable}
\end{figure}
The first example we consider is a coaxial cable, see Figure~\ref{fig:coax_cable}. The geometry consists of three domains, the inner wire $\Omega_\text{I}$ depicted in gray, an area $\Omega_\text{II}$ filled with air in white and the outer tube $\Omega_\text{III}$ in light gray. The inner wire and the outer tube carry the source current $I_\text{S}$, respectively $-I_\text{S}$ which we assume to be homogeneously distributed over the faces. 
We further assume the permeability of the inner wire to be linear, i.e. $\vec{B} = \mu_\text{I} \vec{H}$, whereas the permeability of the outer tube is assumed to be nonlinear, following the Bauer model \textcolor{red}{cite, figure and parameter}. The source current $I_\text{S}$ is considered constant over time, reduces the problem to a magneto-static field problem.

The governing equations are Amp\`{e}re's and Gauss' law, reading
\begin{align}
	\nabla \times \vec{H} &= \vec{J}_\text{I} \quad \text{in~} \Omega_\text{I}, \\
	\nabla \times \vec{H} &= I_\text{S} \quad \text{in~} \Omega_\text{II}, \\
	\nabla \times \vec{H} &= \vec{J}_\text{III} + I_\text{S} \quad \text{in~} \Omega_\text{III}, \\
	\nabla \cdot \vec{B} &= 0 \quad \text{in~}  \Omega,
	\label{eq:amp_gauss}
\end{align}
with boundary conditions
\begin{equation}
	\vec{n} \times \vec{A} = 0 \quad \text{on~} \partial \Omega_\text{III},
\end{equation}
where $\vec{H}$ is the magnetic field strength, $\vec{B}$ is the magnetic flux density, $\vec{A}$ is the magnetic vector potential, $\vec{n}$ denotes the outer normal, $\vec{J}_\text{I}$, $\vec{J}_\text{III}$ are the source current densities in the inner wire and the outer tube.

To solve \eqref{eq:amp_gauss} we also need material information to connect $\vec{B}$ and $\vec{H}$. This information is at hand in form of a data set $\mathcal{D}$, containing corresponding measured $BH$-pairs, i.e.
\begin{equation}
	\mathcal{D} = \left\{(\vec{B}_1,\vec{H}_1),(\vec{B}_2,\vec{H}_2),\dots, (\vec{B}_N,\vec{H}_N)\right\}.
\end{equation}
Thus, the set $\mathcal{D} \in \mathbb{R}^{N\times N \times N \times N}$ is a four dimensional phase space.
In contrast to traditional methods, we do not seek to model the material relation between $\vec{B}$ and $\vec{H}$ explicitly. Instead, we solve the boundary value problem \eqref{eq:amp_gauss} directly with the material data.

\subsection{Brute force minimization}
In this case the distance function was solved with a brute force approach. This approaches scales with $\mathcal{O}(dN^2)$, where $d$ denotes the dimension ($2$ in our case). Table~\ref{tab:iterations_brute_force} shows the number of iterations for an increasing data set.

\begin{table}[htb]
	\centering
	\caption{Iteration steps until convergence} 
	%	\ra{1.3}
	\centering
	\raisebox{\depth}{\begin{tabular}[htbp]{@{}lrrrr@{}}
			\toprule
			data points     & $10^2$ & $10^3$ & $10^4$ & $10^5$  \\
			iteration steps & $85$   & $549$  & $2242$ & ?\\
			\bottomrule
	\end{tabular}}
	\label{tab:iterations_brute_force}
\end{table}


\begin{figure}[htb]
    \centering
    \subfigure[$N=10^2$]{\includegraphics[width=0.24\textwidth]{figures/coax_cable/1e2.pdf}} 
    \subfigure[$N=10^3$]{\includegraphics[width=0.24\textwidth]{figures/coax_cable/1e3.pdf}} 
    \subfigure[$N=10^4$]{\includegraphics[width=0.24\textwidth]{figures/coax_cable/1e4.pdf}}
    \subfigure[$N=10^5$]{\includegraphics[width=0.24\textwidth]{figures/coax_cable/1e2.pdf}}
    \caption{$BH$-curve for increasing number of measurement points $N$. \textcolor{blue}{Blue} stars shows the final $BH$-pairs, fulfilling Amp\`{e}re's and Gausss' law. The \textcolor{orange}{orange} circles show the measurment data, whereas the \textcolor{green}{green} crosses show the chosen $BH$-pairs determined by the distance function. The algorithm performed until convergence.}
    \label{fig:BH_curves_brute_force}
\end{figure}

\begin{figure}[htb]
	\centering
	\subfigure[$N=10^2$]{\includegraphics[width=0.24\textwidth]{figures/coax_cable/1e2_H.pdf}} 
	\subfigure[$N=10^3$]{\includegraphics[width=0.24\textwidth]{figures/coax_cable/1e3_H.pdf}} 
	\subfigure[$N=10^4$]{\includegraphics[width=0.24\textwidth]{figures/coax_cable/1e4_H.pdf}}
	\subfigure[$N=10^5$]{\includegraphics[width=0.24\textwidth]{figures/coax_cable/1e2_H.pdf}}
	\caption{magnetic field strength $H$ for increasing number of measurement points $N$}
	\label{fig:H_brute_force}
\end{figure}

==> coefficient.tex <==
The data-driven algorithm is highly sensitive towards the numerical constant $\widetilde{\nu}$. In particular for sharp material curves, e.g. soft-magnetic material, it is difficult to choose a constant for the whole domain. For example, if we take only the steep gradient at the beginning into account, we receive a relatively high $\widetilde{\mu}$, which is not practical for the saturation part. One could instead, take an average $\widetilde{\mu}$ over all data points, i.e. for one direction
\begin{equation}
	\widetilde{\mu} = \frac{1}{N-1}\sum_{n=1}^{N-1}\frac{B_{n+1} - B_{n}}{H_{n+1} - H_{n}}.
\end{equation}
However, for soft-magnetic material, this still results in unsatisfying results, see Figure~\ref{fig:test_coeff_1e2_samples} left.

To solve that issue, we apply a local constant $\widetilde{\mu}_e$ per element. The results are shown in Figure~\ref{fig:test_coeff_1e2_samples} right.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.47\textwidth]{figures/tests_on_coefficient/dd_nl.png} 
		\hfill
		\includegraphics[width=0.47\textwidth]{figures/tests_on_coefficient/dd_nl_local.png} 
	\end{center} %% end center before the caption
	\caption{\textcolor{blue}{blue points} show the temporal solution, \textcolor{green}{green crosses } the new solution after applying the distance function and \textcolor{orange}{orange circles} the data points. The left plot show the results for the standard approach, the right plot for an approach with local $\nu_\textrm{r}$ } 
	\label{fig:test_coeff_1e2_samples}
\end{figure}

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.49\textwidth]{figures/tests_on_coefficient/Blocal.png} 
		\hfill
		\includegraphics[width=0.49\textwidth]{figures/tests_on_coefficient/mulocal.png} 
	\end{center} 
	\caption{Left: magnetic flux density $\mathbf{B}$. Right: Local $\widetilde{\mu}_z$ in the iron core.}
\end{figure}



